Machine Learning for QoS Prediction in Vehicular Communication: Challenges and Solution Approaches

As cellular networks evolve towards the 6th generation, machine learning is seen as a key enabling technology to improve the capabilities of the network. Machine learning provides a methodology for predictive systems, which can make networks become proactive. This proactive behavior of the network can be leveraged to sustain, for example, a specific quality of service requirement. With predictive quality of service, a wide variety of new use cases, both safety- and entertainment-related, are emerging, especially in the automotive sector. Therefore, in this work, we consider maximum throughput prediction enhancing, for example, streaming or high-definition mapping applications. We discuss the entire machine learning workflow highlighting less regarded aspects such as the detailed sampling procedures, the in-depth analysis of the dataset characteristics, the effects of splits in the provided results, and the data availability. Reliable machine learning models need to face a lot of challenges during their lifecycle. We highlight how confidence can be built on machine learning technologies by better understanding the underlying characteristics of the collected data. We discuss feature engineering and the effects of different splits for the training processes, showcasing that random splits might overestimate performance by more than twofold. Moreover, we investigate diverse sets of input features, where network information proved to be most effective, cutting the error by half. Part of our contribution is the validation of multiple machine learning models within diverse scenarios. We also use explainable AI to show that machine learning can learn underlying principles of wireless networks without being explicitly programmed. Our data is collected from a deployed network that was under full control of the measurement team and covered different vehicular scenarios and radio environments.

==> figures/palai10_n.tex <==
\begin{figure}[tbp]
\begin{center}
\begin{tikzpicture}
\begin{axis}[
	xmin = 1.5, xmax = 20.5,
    %ymin=0.0, ymax=3,
    ylabel = Mean absolute error in Mbit/s,
    xlabel = Rolling window size,
    width=\wFig, height=\hFig, grid=both,
	%legend style={row sep=-0.07cm, inner ysep = 0cm, at={(0.992,0.984)}, anchor=north east},
	xlabel shift = -3 pt, ylabel shift = -4 pt, label style={font=\scriptsize}, tick label style={font=\scriptsize}
    ]
% median
%\addplot+[solid,red,mark=None] table [x=lag_in_seconds, y=density, col sep=comma] {data/handover_lag_density.csv};
    \addplot+[plot_color1,mark=None,semithick]%
    table [x=window, y=mean_absolute_error, col sep=comma] {data/rolling_EMD_DL.csv};
    \addplot+[plot_color2,mark=None,semithick]%
    table [x=window, y=mean_absolute_error, col sep=comma] {data/rolling_MDNET_DL.csv};
    \addplot+[plot_color3,mark=None,semithick]%
    table [x=window, y=mean_absolute_error, col sep=comma] {data/rolling_DEVNET_DL.csv};
    \addplot+[plot_color4,mark=None,semithick]%
    table [x=window, y=mean_absolute_error, col sep=comma] {data/rolling_FULL_DL.csv};
    \legend{\scriptsize{EMD}, \scriptsize{MDNET}, \scriptsize{DEVNET}, \scriptsize{FULL}}
    \end{axis}
\end{tikzpicture}
\end{center}
\vspace*{-3mm}%
\caption{Rolling window response variable.}
\label{fig::rolling_win_y}
%\vspace*{-3.5mm}
\end{figure}

==> tables/MeasurementScenarios.tex <==
%\begin{table}[htbp]
%\centering
%\caption{The different measurement parameters, Raja, Alex}
%\label{tab:CapturedData}
%\begin{tabular}{ll}
%Parameter & Description \\
%Device to Cloud & ... \\
%Device to Device &   Radio Conditions  \\
%Data Generation         & Geographical Location  \\
%Driving schemes& \\
%Type of Measurement  &.. \\
%Protocol &.. \\
%Moving and Stationary & \\
%Propagation Area & \\
%Interference & \\
%\end{tabular}
%\end{table}
